Objective-aware Traffic Simulation via Inverse Reinforcement Learning

Traffic simulators act as an essential component in the operating and planning of transportation systems. Conventional traffic simulators usually employ a calibrated physical car-following model to describe vehicles' behaviors and their interactions with traffic environment. However, there is no universal physical model that can accurately predict the pattern of vehicle's behaviors in different situations. A fixed physical model tends to be less effective in a complicated environment given the non-stationary nature of traffic dynamics. In this paper, we formulate traffic simulation as an inverse reinforcement learning problem, and propose a parameter sharing adversarial inverse reinforcement learning model for dynamics-robust simulation learning. Our proposed model is able to imitate a vehicle's trajectories in the real world while simultaneously recovering the reward function that reveals the vehicle's true objective which is invariant to different dynamics. Extensive experiments on synthetic and real-world datasets show the superior performance of our approach compared to state-of-the-art methods and its robustness to variant dynamics of traffic.

==> LearnSim/implementation.tex <==
\section{Implementation}

\subsection{Simulation Environment}

\nop{It is required to build an environment that controls the movement of vehicles, outputs the system states, and generates the simulated trajectories. }
We created an OpenAI Gym\footnote{https://gym.openai.com/} environment as our simulation environment based on the a traffic simulator called CityFlow\cite{zhang2019cityflow}. This CityFlow based environment is able to provide multiple control APIs that allow us to obtain observations and give direct controls to each vehicle in system. The interaction between learned policy and the simulation environment is shown in Figure \ref{fig:environment}. At each time step, for a certain vehicle, a state representation is generated from the environment. The policy will determine the best action (i.e., next step speed) according to the state and conduct it on the environment. 

\nop{
The simulation environment is initiated with a road network, traffic flow, and a signal plan. The road network includes information of intersections, roads, and length of each lane. The traffic flow provides the track of each vehicle, as well as the time and location it enters the system. The traffic signal plan gives the phase of traffic light for each intersection. In our experiment detailed in Section \ref{sec:experiment}, all these information is sampled from real-world road network and traffic records.}


\subsection{Network Architectures}

For the discriminator of \ours, we use a two-layer fully connected network with 32 units to represent the reward $\hat{r}_\theta$ and the shaping term $h_\phi$. For the policy, we use a two-layer fully connected network with 32 units each layer. The policy network outputs the distribution parameters for a Beta distribution, and the action will be sampled from this distribution.

\nop{For all other learning based methods in Section \ref{sec:experiment}, we use neural networks in similar sizes and structures to represent each model component.
}

Our implementation details can be accessed online.  \footnote{\url{https://www.dropbox.com/sh/os4zqr7paq6bil2/AAAJEJEbkWfN8zWCCRbh2bmra?dl=0}}
Some of the key hyperparameters are shown in Table~\ref{tab:hyper}.
\begin{table}[htp]
    \centering
    \caption{Summary of hyperparameters}
    \begin{tabular}{ll}
    \toprule
    \textbf{Hyperparameters}     & \textbf{Value}  \\
    \midrule
    Update period & 50 timesteps \\
    Discriminator update epoch & 5 \\
    Generator (policy) update epoch & 10 \\
    Batch size & 64\\
    Learning rate $\alpha$ & 0.001\\
    \bottomrule
    \end{tabular}
    \label{tab:hyper}
\end{table}

==> LearnSim/keyword.tex <==

\keywords{Microscopic traffic simulation, learning to simulate, inverse reinforcement learning}

==> LearnSim/reference.tex <==
\bibliographystyle{LearnSim/lib/ijcai21.sty}
  \bibliography{bibfile}
